MM-Align: Learning Optimal Transport-based Alignment Dynamics for Fast and Accurate Inference on Missing Modality Sequences

Existing multimodal tasks mostly target at the complete input modality setting, i.e., each modality is either complete or completely missing in both training and test sets. However, the randomly missing situations have still been underexplored. In this paper, we present a novel approach named MM-Align to address the missing-modality inference problem. Concretely, we propose 1) an alignment dynamics learning module based on the theory of optimal transport (OT) for indirect missing data imputation; 2) a denoising training algorithm to simultaneously enhance the imputation results and backbone network performance. Compared with previous methods which devote to reconstructing the missing inputs, MM-Align learns to capture and imitate the alignment dynamics between modality sequences. Results of comprehensive experiments on three datasets covering two multimodal tasks empirically demonstrate that our method can perform more accurate and faster inference and relieve overfitting under various missing conditions.

==> tables/mosei_avg.tex <==
\renewcommand{\arraystretch}{1.005}
\begin{table}[ht]
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l*{1}{|c c | c c}}
        \toprule
        % \multicolumn{4}{c|}{T $\rightarrow$ V} & \multicolumn{4}{c|}{V$\rightarrow$A}  & \multicolumn{4}{c}{A$\rightarrow$T}   \\
        % \cline{2-13}
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Setting A} & \multicolumn{2}{c}{Setting B} \\
         \cline{2-5}
         ~ & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$}  \\
        \midrule
        LB & 0.791 & 67.2 & 0.791 & 67.2  \\
        UB & 0.645 & 80.6 & 0.645 & 80.6  \\
        \cline{1-5}
        MFM & 0.773 & 68.0 & 0.764 & 68.5 \\
        SMIL & 0.780 & 68.4 & 0.774 & 68.1  \\
        Modal-Trans & 0.764 & 69.8 & 0.761 & 70.2 \\
        \cline{1-5} 
        MM-Align & \textbf{0.757} & \textbf{70.8} & \textbf{0.754} & \textbf{71.2} \\
        \bottomrule
        \end{tabular}
    }
    \caption{Results on the CMU-MOSEI dataset ($p=10$). The reported values are the average performance of six modality pairs (including order) under different setting. Notations share the same meaning as the last table.}
    \label{table:mosei}
\end{table}



==> tables/mosi_and_mosei_main.tex <==
\renewcommand{\arraystretch}{1.000}
\begin{table*}[ht]
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l*{4}{|c c | c c}}
        \toprule
        \multirow{4}{*}{Method} & \multicolumn{8}{c|}{MOSI} & \multicolumn{8}{c}{MOSEI} \\
        \cline{2-17}
       ~ & \multicolumn{2}{c|}{Setting A} & \multicolumn{2}{c|}{Setting B} & \multicolumn{2}{c|}{Setting A} & \multicolumn{2}{c|}{Setting B} & \multicolumn{2}{c|}{Setting A} & \multicolumn{2}{c|}{Setting B} & 
       \multicolumn{2}{c|}{Setting A} & \multicolumn{2}{c}{Setting B} \\
       \cline{2-17}
        ~ & \multicolumn{4}{c|}{T $\rightarrow$ V} & \multicolumn{4}{c|}{V$\rightarrow$T}  & \multicolumn{4}{c|}{T$\rightarrow$V}  & \multicolumn{4}{c}{V$\rightarrow$T}  \\
        \cline{2-17}
         ~ & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$}  & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} \\
        \midrule
        LB & 1.242 & 68.6 & 1.242 & 68.6 & 1.442 & 46.4 & 1.442 & 46.4 & 0.687 & 77.4 & 0.687 & 77.4 & 0.836 & 61.3 & 0.836 & 61.3 \\
        UB & 1.019 & 77.7 & 1.019 & 77.7 & 1.019 & 77.7 & 1.019 & 77.7 & 0.615 & 81.3 & 0.615 & 81.3 & 0.615 & 81.3 & 0.615 & 81.3 \\
        % \cline{1-17}
        \midrule
        MFM & 1.103 & 71.0 & 1.093 & 73.2 & 1.446 & 45.5 & 1.429 & 48.3 & 0.658 & 79.2 & 0.645 & 80.0 & 0.821 & 62.0 & 0.817 & 61.7 \\
        SMIL & 1.073 & 74.2 & 1.052 & 75.3 & 1.448 & 44.2 & 1.447 & 48.9 & 0.680 & 78.3 & 0.648 & 78.5 & 0.820 & 63.1 & 0.816 & 63.5 \\
        Modal-Trans & 1.052 & 75.5 & 1.041 & 75.8 & 1.429 & 50.1 & 1.424 & 51.9 & 0.645 & 79.6 & 0.647 & 79.6 & 0.817 & 64.9 & 0.814 & 65.7 \\
        \midrule
        MM-Align & \textbf{1.028} & \textbf{76.9} & \textbf{1.027} & \textbf{77.0} & \textbf{1.415} & \textbf{52.7} & \textbf{1.410} & \textbf{53.4} & \textbf{0.637} & \textbf{80.8} & \textbf{0.638} & \textbf{81.1} & \textbf{0.812}$^\natural$ & \textbf{65.2}$^\natural$ & \textbf{0.807} & \textbf{66.9} \\
        \midrule
        \multirow{2}{*}{} & 
        \multicolumn{4}{c|}{V $\rightarrow$ A} & \multicolumn{4}{c|}{A$\rightarrow$V}  & \multicolumn{4}{c|}{V$\rightarrow$A} & \multicolumn{4}{c}{A$\rightarrow$V} \\
         \cline{2-17}
         ~ & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$}  \\
        \midrule
        LB & 1.442 & 46.4 & 1.442 & 46.4 & 1.440 & 42.2 & 1.440 & 42.2 & 0.836 & 61.3 & 0.836 & 61.3 & 0.851 & 62.9 & 0.851 & 62.9 \\
        UB & 1.413 & 57.8 & 1.413 & 57.8 & 1.413 & 57.8 & 1.413 & 57.8 & 0.707 & 79.5 & 0.707 & 79.5 & 0.707 & 79.5 & 0.707 & 79.5 \\
        \midrule
        MFM & 1.456 & 43.5 & 1.452 & 43.9 & 1.454 & 42.2 & 1.455 & 42.2 & 0.827 & 60.7 & 0.818 & 61.9 & 0.842 & 62.7 & 0.838 & 63.9 \\
        SMIL & 1.442 & 45.9 & 1.438 & 46.5 & 1.442 & 45.9 & 1.438 & 47.3 & 0.819 & 64.3 & 0.816 & 63.6 & 0.838 & 63.2 & 0.841 & 62.4 \\
        Modal-Trans & 1.428 & 49.4 & 1.425 & 49.7 & 1.439 & 47.1 &1.442 & 48.3 & 0.818 & 64.7 & 0.815 & 65.4 & 0.832 & 64.6 & 0.823 & 65.3 \\
        \midrule
        MM-Align & \textbf{1.416} & \textbf{52.0} & \textbf{1.411} & \textbf{53.0} & \textbf{1.427} & \textbf{49.9} & \textbf{1.426} & \textbf{50.7} & \textbf{0.811} & \textbf{65.9} & \textbf{0.808} & \textbf{66.2} & \textbf{0.822} & \textbf{65.4} & \textbf{0.818}$^\natural$ & \textbf{65.7}$^\natural$ \\
        \midrule
        \multirow{2}{*}{} & 
        \multicolumn{4}{c|}{A $\rightarrow$ T} & \multicolumn{4}{c|}{T$\rightarrow$A}  & \multicolumn{4}{c|}{A $\rightarrow$T} & \multicolumn{4}{c}{T$\rightarrow$A} \\
         \cline{2-17}
         ~ & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$} & \textbf{MAE$\downarrow$} & \textbf{Acc-2$\uparrow$}  \\
        \midrule
        LB & 1.440 & 42.2 & 1.440 & 42.2 & 1.242 & 68.6 & 1.242 & 68.6 & 0.851 & 62.9 & 0.851 & 62.9 & 0.687 & 77.4 & 0.687 & 77.4 \\
        UB & 1.081 & 75.8 & 1.081 & 75.8 & 1.081 & 75.8 & 1.081 & 75.8 & 0.613 & 80.9 & 0.613 & 80.9 & 0.613 & 80.9 & 0.613 & 80.9 \\
        \midrule
        MFM & 1.447 & 42.2 & 1.454 & 42.2 & 1.078 & 72.9 & 1.082 & 73.7 & 0.830 & 64.5 & 0.830 & 63.6 & 0.658 & 79.1 & 0.645 & 79.7 \\
        SMIL & 1.447 & 43.3 & 1.439 & 45.4 & 1.060 & 75.5 & 1.089 & 74.9 & 0.840 & 62.9 & 8.839 & 63.0 & 0.684 & 78.5 & 0.684 & 77.4\\
        Modal-Trans & 1.435 & 48.7 & 1.432 & 48.7 & 1.052 & 75.2 & 1.073 & 74.3 & 0.827 & 64.9 & 0.823 & 65.6 & 0.643 & 79.9 & 0.644 & 79.6 \\
        \midrule
        MM-Align & \textbf{1.426}$^\natural$ & \textbf{51.5} & \textbf{1.414} & \textbf{52.0} & \textbf{1.028} & \textbf{76.8} & \textbf{1.032} & \textbf{76.6} & \textbf{0.824}$^\natural$ & \textbf{65.3} & \textbf{0.817} & \textbf{66.3}$^\natural$ & \textbf{0.635} & \textbf{81.0} & \textbf{0.637} & \textbf{80.9} \\
        \bottomrule
    \end{tabular}
    }
    \caption{Results on the CMU-MOSI and CMU-MOSEI dataset~($p=10\%$). 
    The results are the average of five runs. 
    ``A $\to$ B'' represents the imputation from the complete modality A to the missing modality B at test time. $\natural$: results of our model are significantly better than the highest baselines but NOT passed the paired t-test (p-value $<$ 0.05).}
    \label{table:mosi_and_mosei}
\end{table*}


